Adaptive Generation of Unrestricted Adversarial Inputs

Neural networks are vulnerable to adversarially-constructed perturbations of their inputs. Most research so far has considered perturbations of a fixed magnitude under some $l_p$ norm. Although studying these attacks is valuable, there has been increasing interest in the construction of (and robustness to) unrestricted attacks, which are not constrained to a small and rather artificial subset of all possible adversarial inputs. We introduce a novel algorithm for generating such unrestricted adversarial inputs which, unlike prior work, is adaptive: it is able to tune its attacks to the classifier being targeted. It also offers a 400-2,000x speedup over the existing state of the art. We demonstrate our approach by generating unrestricted adversarial inputs that fool classifiers robust to perturbation-based attacks. We also show that, by virtue of being adaptive and unrestricted, our attack is able to defeat adversarial training against it.

==> exapmles_table_MIxTrain.tex <==
\begin{minipage}[t]{0.48\linewidth}\centering

    \hspace{1cm} Target label 
    \vspace{2mm}

    \renewcommand{\arraystretch}{0.2} % whitespace between rows (multiplicative factor)
    \begin{tabular}{cr*{11}{c}}
    & & 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & \hspace{0.7mm} None \vspace{1mm} \\
& 0 \hspace{2mm} & \hspace{15mm}& \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/0/1/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/0/2/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/0/3/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/0/4/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/0/5/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/0/6/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/0/7/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/0/8/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/0/9/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/0/-1/1.png} \\
& 1 \hspace{2mm} & \hspace{15mm}& \hspace{15mm}& \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/1/2/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/1/3/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/1/4/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/1/5/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/1/6/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/1/7/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/1/8/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/1/9/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/1/-1/1.png} \\
\parbox[t]{4mm}{\multirow{11}{*}{\rotatebox[origin=c]{90}{Intended true label}}} & 2 \hspace{2mm} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/2/0/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/2/1/1.png} & \hspace{15mm}& \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/2/3/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/2/4/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/2/5/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/2/6/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/2/7/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/2/8/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/2/9/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/2/-1/1.png} \\
& 3 \hspace{2mm} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/3/0/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/3/1/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/3/2/1.png} & \hspace{15mm}& \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/3/4/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/3/5/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/3/6/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/3/7/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/3/8/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/3/9/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/3/-1/1.png} \\
& 4 \hspace{2mm} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/4/0/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/4/1/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/4/2/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/4/3/1.png} & \hspace{15mm}& \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/4/5/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/4/6/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/4/7/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/4/8/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/4/9/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/4/-1/1.png} \\
& 5 \hspace{2mm} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/5/0/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/5/1/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/5/2/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/5/3/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/5/4/1.png} & \hspace{15mm}& \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/5/6/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/5/7/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/5/8/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/5/9/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/5/-1/1.png} \\
& 6 \hspace{2mm} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/6/0/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/6/1/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/6/2/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/6/3/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/6/4/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/6/5/1.png} & \hspace{15mm}& \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/6/7/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/6/8/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/6/9/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/6/-1/1.png} \\
& 7 \hspace{2mm} & \hspace{15mm}& \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/7/1/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/7/2/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/7/3/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/7/4/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/7/5/1.png} & \hspace{15mm}& \hspace{15mm}& \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/7/8/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/7/9/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/7/-1/1.png} \\
& 8 \hspace{2mm} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/8/0/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/8/1/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/8/2/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/8/3/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/8/4/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/8/5/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/8/6/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/8/7/1.png} & \hspace{15mm}& \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/8/9/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/8/-1/1.png} \\
& 9 \hspace{2mm} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/9/0/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/9/1/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/9/2/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/9/3/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/9/4/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/9/5/1.png} & \hspace{15mm}& \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/9/7/1.png} & \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/9/8/1.png} & \hspace{15mm}& \includegraphics[width=4.8mm]{adv_samples/individual/finetuned/mixtrain0/9/-1/1.png} \\
    \end{tabular}
    \caption{Randomly-selected
    images generated by a finetuned GAN
    to attack the MixTrain 0 locally-robust classifier.
    The computed label given by the classifier
    matches the target label for each image.} 
    \label{generated-samples-the MixTrain 0}
\end{minipage}

==> generated_mixtrain_samples_figure.tex <==

 \pagenumbering{gobble} \begin{figure}[H]
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/A/grid_adversarial_s0_t-1.png}
                \caption{Intended true label `0'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/A/grid_adversarial_s1_t-1.png}
                \caption{Intended true label `1'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/A/grid_adversarial_s2_t-1.png}
                \caption{Intended true label `2'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/A/grid_adversarial_s3_t-1.png}
                \caption{Intended true label `3'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/A/grid_adversarial_s4_t-1.png}
                \caption{Intended true label `4'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/A/grid_adversarial_s5_t-1.png}
                \caption{Intended true label `5'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/A/grid_adversarial_s6_t-1.png}
                \caption{Intended true label `6'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/A/grid_adversarial_s7_t-1.png}
                \caption{Intended true label `7'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/A/grid_adversarial_s8_t-1.png}
                \caption{Intended true label `8'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/A/grid_adversarial_s9_t-1.png}
                \caption{Intended true label `9'.} 
            \end{subfigure}
        \medskip
 \caption{Examples of adversarial images generated by a GAN finetuned to perform an untargeted attack for MixTrain model A.}
\end{figure}


 \pagenumbering{gobble} \begin{figure}[H]
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/B/grid_adversarial_s0_t-1.png}
                \caption{Intended true label `0'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/B/grid_adversarial_s1_t-1.png}
                \caption{Intended true label `1'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/B/grid_adversarial_s2_t-1.png}
                \caption{Intended true label `2'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/B/grid_adversarial_s3_t-1.png}
                \caption{Intended true label `3'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/B/grid_adversarial_s4_t-1.png}
                \caption{Intended true label `4'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/B/grid_adversarial_s5_t-1.png}
                \caption{Intended true label `5'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/B/grid_adversarial_s6_t-1.png}
                \caption{Intended true label `6'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/B/grid_adversarial_s7_t-1.png}
                \caption{Intended true label `7'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/B/grid_adversarial_s8_t-1.png}
                \caption{Intended true label `8'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/B/grid_adversarial_s9_t-1.png}
                \caption{Intended true label `9'.} 
            \end{subfigure}
        \medskip
 \caption{Examples of adversarial images generated by a GAN finetuned to perform an untargeted attack for MixTrain model B.}
\end{figure}


 \pagenumbering{gobble} \begin{figure}[H]
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/C/grid_adversarial_s0_t-1.png}
                \caption{Intended true label `0'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/C/grid_adversarial_s1_t-1.png}
                \caption{Intended true label `1'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/C/grid_adversarial_s2_t-1.png}
                \caption{Intended true label `2'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/C/grid_adversarial_s3_t-1.png}
                \caption{Intended true label `3'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/C/grid_adversarial_s4_t-1.png}
                \caption{Intended true label `4'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/C/grid_adversarial_s5_t-1.png}
                \caption{Intended true label `5'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/C/grid_adversarial_s6_t-1.png}
                \caption{Intended true label `6'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/C/grid_adversarial_s7_t-1.png}
                \caption{Intended true label `7'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/C/grid_adversarial_s8_t-1.png}
                \caption{Intended true label `8'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/C/grid_adversarial_s9_t-1.png}
                \caption{Intended true label `9'.} 
            \end{subfigure}
        \medskip
 \caption{Examples of adversarial images generated by a GAN finetuned to perform an untargeted attack for MixTrain model C.}
\end{figure}


 \pagenumbering{gobble} \begin{figure}[H]
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/D/grid_adversarial_s0_t-1.png}
                \caption{Intended true label `0'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/D/grid_adversarial_s1_t-1.png}
                \caption{Intended true label `1'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/D/grid_adversarial_s2_t-1.png}
                \caption{Intended true label `2'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/D/grid_adversarial_s3_t-1.png}
                \caption{Intended true label `3'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/D/grid_adversarial_s4_t-1.png}
                \caption{Intended true label `4'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/D/grid_adversarial_s5_t-1.png}
                \caption{Intended true label `5'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/D/grid_adversarial_s6_t-1.png}
                \caption{Intended true label `6'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/D/grid_adversarial_s7_t-1.png}
                \caption{Intended true label `7'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/D/grid_adversarial_s8_t-1.png}
                \caption{Intended true label `8'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/mixtrain/D/grid_adversarial_s9_t-1.png}
                \caption{Intended true label `9'.} 
            \end{subfigure}
        \medskip
 \caption{Examples of adversarial images generated by a GAN finetuned to perform an untargeted attack for MixTrain model D.}
\end{figure}


==> generated_samples_figure.tex <==

 \pagenumbering{gobble} \begin{figure}[H]
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s0_t-1.png}
                \caption{Intended true label `0'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s1_t-1.png}
                \caption{Intended true label `1'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s2_t-1.png}
                \caption{Intended true label `2'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s3_t-1.png}
                \caption{Intended true label `3'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s4_t-1.png}
                \caption{Intended true label `4'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s5_t-1.png}
                \caption{Intended true label `5'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s6_t-1.png}
                \caption{Intended true label `6'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s7_t-1.png}
                \caption{Intended true label `7'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s8_t-1.png}
                \caption{Intended true label `8'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s9_t-1.png}
                \caption{Intended true label `9'.} 
            \end{subfigure}
        \medskip
 \caption{Examples of expected-adversarial images generated by a GAN finetuned to perform an untargeted attack on Wong and Kolter's locally-robust classifier network.}
\end{figure}


 \pagenumbering{gobble} \begin{figure}[H]
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s0_t0.png}
                \caption{Intended true label `0'. (Therefore not adversarial.)} 
            \end{subfigure}
        \hspace*{\fill}
                \begin{subfigure}{0.45\textwidth}
                    \caption{No expected-adversarial images were found for intended true label 1.} 
                \end{subfigure}
            \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s2_t0.png}
                \caption{Intended true label `2'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s3_t0.png}
                \caption{Intended true label `3'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s4_t0.png}
                \caption{Intended true label `4'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s5_t0.png}
                \caption{Intended true label `5'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s6_t0.png}
                \caption{Intended true label `6'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s7_t0.png}
                \caption{Intended true label `7'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s8_t0.png}
                \caption{Intended true label `8'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s9_t0.png}
                \caption{Intended true label `9'.} 
            \end{subfigure}
        \medskip
 \caption{Examples of expected-adversarial images generated by a GAN finetuned to target label 0 for Wong and Kolter's locally-robust classifier network.}
\end{figure}


 \pagenumbering{gobble} \begin{figure}[H]
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s0_t1.png}
                \caption{Intended true label `0'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s1_t1.png}
                \caption{Intended true label `1'. (Therefore not adversarial.)} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s2_t1.png}
                \caption{Intended true label `2'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s3_t1.png}
                \caption{Intended true label `3'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s4_t1.png}
                \caption{Intended true label `4'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s5_t1.png}
                \caption{Intended true label `5'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s6_t1.png}
                \caption{Intended true label `6'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s7_t1.png}
                \caption{Intended true label `7'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s8_t1.png}
                \caption{Intended true label `8'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s9_t1.png}
                \caption{Intended true label `9'.} 
            \end{subfigure}
        \medskip
 \caption{Examples of expected-adversarial images generated by a GAN finetuned to target label 1 for Wong and Kolter's locally-robust classifier network.}
\end{figure}


 \pagenumbering{gobble} \begin{figure}[H]
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s0_t2.png}
                \caption{Intended true label `0'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s1_t2.png}
                \caption{Intended true label `1'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s2_t2.png}
                \caption{Intended true label `2'. (Therefore not adversarial.)} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s3_t2.png}
                \caption{Intended true label `3'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s4_t2.png}
                \caption{Intended true label `4'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s5_t2.png}
                \caption{Intended true label `5'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s6_t2.png}
                \caption{Intended true label `6'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s7_t2.png}
                \caption{Intended true label `7'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s8_t2.png}
                \caption{Intended true label `8'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s9_t2.png}
                \caption{Intended true label `9'.} 
            \end{subfigure}
        \medskip
 \caption{Examples of expected-adversarial images generated by a GAN finetuned to target label 2 for Wong and Kolter's locally-robust classifier network.}
\end{figure}


 \pagenumbering{gobble} \begin{figure}[H]
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s0_t3.png}
                \caption{Intended true label `0'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 0.00cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s1_t3.png}
                \caption{Intended true label `1'. These were the only adversarial images found in 100 seconds.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s2_t3.png}
                \caption{Intended true label `2'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s3_t3.png}
                \caption{Intended true label `3'. (Therefore not adversarial.)} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s4_t3.png}
                \caption{Intended true label `4'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s5_t3.png}
                \caption{Intended true label `5'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s6_t3.png}
                \caption{Intended true label `6'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s7_t3.png}
                \caption{Intended true label `7'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s8_t3.png}
                \caption{Intended true label `8'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s9_t3.png}
                \caption{Intended true label `9'.} 
            \end{subfigure}
        \medskip
 \caption{Examples of expected-adversarial images generated by a GAN finetuned to target label 3 for Wong and Kolter's locally-robust classifier network.}
\end{figure}


 \pagenumbering{gobble} \begin{figure}[H]
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s0_t4.png}
                \caption{Intended true label `0'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 0.00cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s1_t4.png}
                \caption{Intended true label `1'. These were the only adversarial images found in 100 seconds.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s2_t4.png}
                \caption{Intended true label `2'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s3_t4.png}
                \caption{Intended true label `3'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s4_t4.png}
                \caption{Intended true label `4'. (Therefore not adversarial.)} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s5_t4.png}
                \caption{Intended true label `5'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s6_t4.png}
                \caption{Intended true label `6'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s7_t4.png}
                \caption{Intended true label `7'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s8_t4.png}
                \caption{Intended true label `8'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s9_t4.png}
                \caption{Intended true label `9'.} 
            \end{subfigure}
        \medskip
 \caption{Examples of expected-adversarial images generated by a GAN finetuned to target label 4 for Wong and Kolter's locally-robust classifier network.}
\end{figure}


 \pagenumbering{gobble} \begin{figure}[H]
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s0_t5.png}
                \caption{Intended true label `0'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s1_t5.png}
                \caption{Intended true label `1'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s2_t5.png}
                \caption{Intended true label `2'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s3_t5.png}
                \caption{Intended true label `3'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s4_t5.png}
                \caption{Intended true label `4'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s5_t5.png}
                \caption{Intended true label `5'. (Therefore not adversarial.)} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s6_t5.png}
                \caption{Intended true label `6'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s7_t5.png}
                \caption{Intended true label `7'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s8_t5.png}
                \caption{Intended true label `8'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s9_t5.png}
                \caption{Intended true label `9'.} 
            \end{subfigure}
        \medskip
 \caption{Examples of expected-adversarial images generated by a GAN finetuned to target label 5 for Wong and Kolter's locally-robust classifier network.}
\end{figure}


 \pagenumbering{gobble} \begin{figure}[H]
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s0_t6.png}
                \caption{Intended true label `0'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s1_t6.png}
                \caption{Intended true label `1'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s2_t6.png}
                \caption{Intended true label `2'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s3_t6.png}
                \caption{Intended true label `3'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s4_t6.png}
                \caption{Intended true label `4'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s5_t6.png}
                \caption{Intended true label `5'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s6_t6.png}
                \caption{Intended true label `6'. (Therefore not adversarial.)} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s7_t6.png}
                \caption{Intended true label `7'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s8_t6.png}
                \caption{Intended true label `8'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s9_t6.png}
                \caption{Intended true label `9'.} 
            \end{subfigure}
        \medskip
 \caption{Examples of expected-adversarial images generated by a GAN finetuned to target label 6 for Wong and Kolter's locally-robust classifier network.}
\end{figure}


 \pagenumbering{gobble} \begin{figure}[H]
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s0_t7.png}
                \caption{Intended true label `0'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 0.00cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s1_t7.png}
                \caption{Intended true label `1'. These were the only adversarial images found in 100 seconds.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s2_t7.png}
                \caption{Intended true label `2'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s3_t7.png}
                \caption{Intended true label `3'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s4_t7.png}
                \caption{Intended true label `4'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s5_t7.png}
                \caption{Intended true label `5'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s6_t7.png}
                \caption{Intended true label `6'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s7_t7.png}
                \caption{Intended true label `7'. (Therefore not adversarial.)} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s8_t7.png}
                \caption{Intended true label `8'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s9_t7.png}
                \caption{Intended true label `9'.} 
            \end{subfigure}
        \medskip
 \caption{Examples of expected-adversarial images generated by a GAN finetuned to target label 7 for Wong and Kolter's locally-robust classifier network.}
\end{figure}


 \pagenumbering{gobble} \begin{figure}[H]
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s0_t8.png}
                \caption{Intended true label `0'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 2.20cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s1_t8.png}
                \caption{Intended true label `1'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s2_t8.png}
                \caption{Intended true label `2'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s3_t8.png}
                \caption{Intended true label `3'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s4_t8.png}
                \caption{Intended true label `4'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s5_t8.png}
                \caption{Intended true label `5'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s6_t8.png}
                \caption{Intended true label `6'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s7_t8.png}
                \caption{Intended true label `7'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s8_t8.png}
                \caption{Intended true label `8'. (Therefore not adversarial.)} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s9_t8.png}
                \caption{Intended true label `9'.} 
            \end{subfigure}
        \medskip
 \caption{Examples of expected-adversarial images generated by a GAN finetuned to target label 8 for Wong and Kolter's locally-robust classifier network.}
\end{figure}


 \pagenumbering{gobble} \begin{figure}[H]
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s0_t9.png}
                \caption{Intended true label `0'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=3cm, clip, trim=0.0cm 0.00cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s1_t9.png}
                \caption{Intended true label `1'. These were the only adversarial images found in 100 seconds.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s2_t9.png}
                \caption{Intended true label `2'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 1.15cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s3_t9.png}
                \caption{Intended true label `3'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s4_t9.png}
                \caption{Intended true label `4'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s5_t9.png}
                \caption{Intended true label `5'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s6_t9.png}
                \caption{Intended true label `6'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s7_t9.png}
                \caption{Intended true label `7'.} 
            \end{subfigure}
        \medskip
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s8_t9.png}
                \caption{Intended true label `8'.} 
            \end{subfigure}
        \hspace*{\fill}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\linewidth, clip, trim=0.0cm 5.30cm 0.0cm 0.0cm]{adv_samples/grid/grid_adversarial_s9_t9.png}
                \caption{Intended true label `9'. (Therefore not adversarial.)} 
            \end{subfigure}
        \medskip
 \caption{Examples of expected-adversarial images generated by a GAN finetuned to target label 9 for Wong and Kolter's locally-robust classifier network.}
\end{figure}

